Enhancing Self-Supervised Fine-Grained Video Object Tracking with Dynamic Memory Prediction

Successful video analysis relies on accurate recognition of pixels across frames, and frame reconstruction methods based on video correspondence learning are popular due to their efficiency. Existing frame reconstruction methods, while efficient, neglect the value of direct involvement of multiple reference frames for reconstruction and decision-making aspects, especially in complex situations such as occlusion or fast movement. In this paper, we introduce a Dynamic Memory Prediction (DMP) framework that innovatively utilizes multiple reference frames to concisely and directly enhance frame reconstruction. Its core component is a Reference Frame Memory Engine that dynamically selects frames based on object pixel features to improve tracking accuracy. In addition, a Bidirectional Target Prediction Network is built to utilize multiple reference frames to improve the robustness of the model. Through experiments, our algorithm outperforms the state-of-the-art self-supervised techniques on two fine-grained video object tracking tasks: object segmentation and keypoint tracking.

==> tables/heat_map.tex <==
% heatmap-figure.tex
% 请确保主文档已加载：
%   \usepackage{pgfplots}
%   \pgfplotsset{compat=1.17}
%   \usepackage{filecontents}



\begin{figure}[htbp]
  \centering
  \begin{tikzpicture}
    \begin{axis}[
      width=0.8\columnwidth,      % 单栏宽度
      height=0.6\columnwidth,  % 高度可根据需求调整
      xlabel={$\delta$}, ylabel={$\theta$},
      title={Tracking Accuracy (\%) for Different $\theta$–$\delta$ Pairs},
      colormap/viridis,
      colorbar,
      point meta min=75.0,
      point meta max=75.6,
      mesh/cols=6,
      mesh/ordering=x varies,
      unbounded coords=jump,
      xtick={0.00,0.05,0.10,0.15,0.20,0.25},
      ytick={0.70,0.75,0.80,0.85,0.90,0.95},
      axis on top,
      enlargelimits=false,
      tick align=inside,
    ]
      \addplot[
        matrix plot*,
        point meta=explicit,
        nodes near coords,
        nodes near coords align={center},
        every node near coord/.style={font=\small},
      ] table[
        x=delta,
        y=theta,
        meta=value,
        col sep=comma
      ] {heatmap-data.csv};
    \end{axis}
  \end{tikzpicture}
  \caption{Heatmap of tracking accuracy (\%) across $\theta$ and $\delta$.}
  \label{fig:theta-delta-heatmap}
\end{figure}

